Rethinking Transfer Learning for Medical Image Classification

Transfer learning (TL) from pretrained deep models is a standard practice in modern medical image classification (MIC). However, what levels of features to be reused are problem-dependent, and uniformly finetuning all layers of pretrained models may be suboptimal. This insight has partly motivated the recent differential TL strategies, such as TransFusion (TF) and layer-wise finetuning (LWFT), which treat the layers in the pretrained models differentially. In this paper, we add one more strategy into this family, called TruncatedTL, which reuses and finetunes appropriate bottom layers and directly discards the remaining layers. This yields not only superior MIC performance but also compact models for efficient inference, compared to other differential TL methods. Our code is available at: https://github.com/sun-umn/TTL

==> tables/3D.tex <==
\begin{table}[!htpb]
\centering
% \begin{adjustbox}{width=\columnwidth,center}
\caption{3D Pulmonary Embolism Classification with different TL strategies.}
% \begin{center}
\setlength{\tabcolsep}{1.0mm}{
%\renewcommand\arraystretch{1.25}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c | c c c c c c }
\toprule
Method&
AUROC$\uparrow$&
AUPRC$\uparrow$ &
Params(M)$\downarrow$ &
MACs(G)$\downarrow$ &
CPU(\textcolor{blue}{s})$\downarrow$ & 
GPU(\textcolor{blue}{s})$\downarrow$ \\
\midrule
%\hline
\midrule


% \midrule
%\hline
{PENet}
&\tabincell{c}{{$0.822 \pm 0.010$}}
&\tabincell{c}{{$0.855 \pm 0.007$}}
&\tabincell{c}{{28.4}}
&\tabincell{c}{\textcolor{red}{$\mb{51.7}$}}
&\tabincell{c}{{1.50}}
&\tabincell{c}{\textcolor{red}{$\mb{1.59}$e-$\mb 2$}}
\\
\cmidrule(l){1-7}
%   \ctoprule(l){1-8}
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=r]{90}{block-wise}}}&
{FTL}
    &\tabincell{c}{{$0.821 \pm 0.010$}}
    &\tabincell{c}{{$0.867 \pm 0.006$}}
    &\tabincell{c}{{47.5}}
    &\tabincell{c}{{66.3}}
    &\tabincell{c}{{1.44}}
    &\tabincell{c}{{1.96e-2}}
\\
\cmidrule(l){1-7}
% &
    {TF-1}
    &\tabincell{c}{{{$0.849 \pm 0.020$}}}
    &\tabincell{c}{{$0.886 \pm 0.017$}}
    &\tabincell{c}{{36.1}}
    &\tabincell{c}{{64.9}}
    &\tabincell{c}{{1.41}}
    &\tabincell{c}{1.93e-2}
\\
\cmidrule(l){2-7}
% &
{LWFT-1}
    &\tabincell{c}{$0.817 \pm 0.005$}
    &\tabincell{c}{$0.855 \pm 0.003$}
    &\tabincell{c}{47.5}
    &\tabincell{c}{{66.3}}
    &\tabincell{c}{{1.44}}
    &\tabincell{c}{{1.96e-2}}
\\
\cmidrule(l){2-7}
% &
    {\textbf{TTL-1}}
    &\tabincell{c}{\textcolor{red}{{$\mathbf{0.854 \pm 0.013}$}}}
    &\tabincell{c}{\textcolor{red}{$\mathbf{0.889 \pm 0.015}$}}
    &\tabincell{c}{\textcolor{red}{$\mb{26.11}$}}
    &\tabincell{c}{{60.17}}
    &\tabincell{c}{{\textcolor{red}{\textbf{1.32}}}}
    &\tabincell{c}{{1.68e-2}}
\\


%%%%%%%%%%%%%%%%%%%%%% layer wise result
\midrule
% \parbox[t]{4mm}{\multirow{4}{*}{\rotatebox[origin=r]{90}{layer-wise}}}&

% \midrule
%\hline
% &
{TF-2}
    &\tabincell{c}{{{$0.849 \pm 0.020$}}}
    &\tabincell{c}{{$0.886 \pm 0.017$}}
    &\tabincell{c}{{36.1}}
    &\tabincell{c}{{64.9}}
    &\tabincell{c}{{1.41}}
    &\tabincell{c}{1.93e-2}
\\
\cmidrule(l){2-7}
% &
{LWFT-2}
    &\tabincell{c}{{{$0.835 \pm 0.038$}}}
    &\tabincell{c}{{$0.870 \pm 0.028$}}
&\tabincell{c}{47.5}
&\tabincell{c}{66.3}
&\tabincell{c}{1.44}
&\tabincell{c}{1.96e-2}
\\
\cmidrule(l){2-7}
% &
    {\textbf{TTL-2(ours)}}
    &\tabincell{c}{\textcolor{red}{{$\mathbf{0.854 \pm 0.013}$}}}
    &\tabincell{c}{\textcolor{red}{$\mathbf{0.889 \pm 0.015}$}}
    &\tabincell{c}{\textcolor{red}{$\mb{26.11}$}}
    &\tabincell{c}{{60.17}}
    &\tabincell{c}{{\textcolor{red}{\textbf{1.32}}}}
    &\tabincell{c}{{1.68e-2}}
\\

\bottomrule
\end{tabular}
}}
\label{tab:penet_comparision}
% \end{center}
% \end{adjustbox}
\end{table}

==> tables/bimcv.tex <==
\
\begin{table}[!htpb]
  \centering
  % \begin{adjustbox}{width=\columnwidth,center}
  \caption{COVID-19 classification with different TL strategies. The best result of each column is colored in \textcolor{red}{\textbf{red}}. $\uparrow$ indicates larger value is better and $\downarrow$ indicates lower value is better. ``-1" means with the block-wise search only, and ``-2" means with the two-stage block-layer hierarchical search. }
  % \begin{center}
  \hspace{5pt}
  \setlength{\tabcolsep}{1.0mm}{
  %\renewcommand\arraystretch{1.25}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{c |c c c c c c }
  \toprule
  Method&
  AUROC$\uparrow$&
  AUPRC$\uparrow$ &
  Params(M)$\downarrow$ &
  MACs(G)$\downarrow$ &
  CPU(ms)$\downarrow$ &
  GPU(ms)$\downarrow$ \\ 
  % \cline{6-7}
  \midrule
  %\hline
  \midrule
  % \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=r]{90}{block-wise}}}&
  
  % \midrule
  %\hline
  {FTL}
  &\tabincell{c}{{$0.849 \pm 0.001$}}
  &\tabincell{c}{{$0.857 \pm 0.003$}}
  &\tabincell{c}{{23.5}}
  &\tabincell{c}{{4.12}}
  &\tabincell{c}{{79.6}}
  &\tabincell{c}{{3.59}}
  \\
  \cmidrule(l){1-7}
  % &
  {TF-1}
  &\tabincell{c}{{$0.856 \pm 0.011$}}
  &\tabincell{c}{{$0.863 \pm 0.012$}}
  &\tabincell{c}{12.9}
  &\tabincell{c}{3.56}
  &\tabincell{c}{{67.0}}
  &\tabincell{c}{{3.55}}
  \\
  \cmidrule(l){2-7}
  % &
  {LWFT-1}
  &\tabincell{c}{{$0.848 \pm 0.002$}}
  &\tabincell{c}{{{$0.861 \pm 0.004$}}}
  &\tabincell{c}{{23.5}}
  &\tabincell{c}{4.12}
  &\tabincell{c}{{76.9}}
  &\tabincell{c}{3.59}
  \\
  \cmidrule(l){2-7}
  % &
  {\textbf{TTL-1}}
  &\tabincell{c}{$0.851 \pm 0.002$}
  &\tabincell{c}{$0.860 \pm 0.002$}
  &\tabincell{c}{8.55}
  &\tabincell{c}{3.31}
  &\tabincell{c}{59.7}
  &\tabincell{c}{3.19}
  \\
  %%%%%%%%%%%%%%%%%%%%%% layer wise result
  \midrule
  {TF-2}
  &\tabincell{c}{$0.856 \pm 0.011$}
  &\tabincell{c}{$0.863 \pm 0.012$}
  &\tabincell{c}{12.9}
  &\tabincell{c}{3.56}
  &\tabincell{c}{{72.7}}
  &\tabincell{c}{{3.56}}
  \\
  \cmidrule(l){2-7}
  % &
  LWFT-2
  &\tabincell{c}{{{$0.853 \pm 0.005$}}}
  &\tabincell{c}{{$0.861 \pm 0.001$}}
  &\tabincell{c}{{23.5}}
  &\tabincell{c}{{4.12}}
  &\tabincell{c}{{79.7}}
  &\tabincell{c}{3.56}
  \\
  \cmidrule(l){2-7}
  % &
  {\textbf{TTL-2 (ours)}}
  &\tabincell{c}{\textcolor{red}{{$\mathbf{0.861 \pm 0.013}$}}}
  &\tabincell{c}{\textcolor{red}{$\mathbf{0.871 \pm 0.008}$}}
  &\tabincell{c}{\textcolor{red}{\textbf{6.31}}}
  &\tabincell{c}{\textcolor{red}{\textbf{2.87}}}
  &\tabincell{c}{{\textcolor{red}{\textbf{53.1}}}}
  &\tabincell{c}{\textcolor{red}{\textbf{2.97}}}
  \\
  
  \bottomrule
  \end{tabular}
  }}
  \label{tab:bimcv_comparision_method}
  % \end{center}
  % \end{adjustbox}
\end{table}




==> tables/lung.tex <==
    \begin{table}[!htbp]
        \centering
        % \begin{adjustbox}{width=\columnwidth,center}
        \caption{2D lung segmentation with TTL. The best result of each column is colored in \textcolor{red}{\textbf{red}}. $\uparrow$ indicates larger value is better and $\downarrow$ indicates lower value is better.}
        \label{tab:lung_segmentation}
        % \begin{center}
        \setlength{\tabcolsep}{2.0mm}{
        %\renewcommand\arraystretch{1.25}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c| c c c c c c}
        \toprule
         Method &
        Dice Coef $\uparrow$ &
        Jaccard index $\uparrow$ &
        Params(M) $\downarrow$ &
        MACs(G) $\downarrow$ &
        CPU(ms) $\downarrow$ & 
        GPU(ms) $\downarrow$\\
        \midrule
        \hline
        {FTL}
        & $0.968 \pm 0.029$
        & $0.940 \pm \small{0.051}$
        & $24.4$
        & $5.93$
        & $121$
        & $11.8$
        \\
        %\cmidrule(l){1-1}
        \midrule
        %\hline
        {\textbf{TTL\_B1(Ours)}}
        & $0.970 \pm 0.029$
        & $0.941 \pm 0.052$
        % &\tabincell{c}{\textcolor{red}{\mathbf{21.3}}}
        &\textcolor{red}{$\mb 21.3$}
        &\textcolor{red}{$\mb 1.68$}
        &\textcolor{red}{$\mb 47.8$}
        &\textcolor{red}{$\mb 7.05$}
        \\
        \cmidrule(l){2-7}
        {\textbf{TTL\_B2(Ours)}}
        &\textcolor{red}{$\mathbf{0.972 \pm 0.027}$}
        &\textcolor{red}{$\mathbf{0.946 \pm 0.047}$}
        &$21.5$
        &$3.02$
        &$68.7$
        &$8.50$
        \\
        \cmidrule(l){2-7}
        {\textbf{TTL\_B3(Ours)}}
        & $0.968 \pm 0.029$
        & $0.939 \pm 0.051$
        &$22.1$
        &$4.82$
        &$95.6$
        &$10.6$
        \\
        \bottomrule
        \end{tabular}
        }}
        \end{table}

==> tables/mitotic.tex <==
\begin{table}[!htpb]
\centering
% \begin{adjustbox}{width=\columnwidth,center}
\caption{Mitotic cells classification with different TL strategies.}
% \begin{center}
\setlength{\tabcolsep}{1.0mm}{
%\renewcommand\arraystretch{1.25}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c | c c c c c c c}
\toprule
% &
Method&
AUROC$\uparrow$ &
AUPRC$\uparrow$ &
Params(M)$\downarrow$ &
MACs(G)$\downarrow$ &
CPU(ms)$\downarrow$ & 
GPU(ms)$\downarrow$ \\
% \cline{7-8}
\midrule
%\hline
\midrule
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=r]{90}{block-wise}}}&

% \midrule
%\hline
{FTL}
&\tabincell{c}{$0.925 \pm 0.003$}
&\tabincell{c}{$0.917 \pm 0.003$}
&\tabincell{c}{23.5}
&\tabincell{c}{4.12}
&\tabincell{c}{80.1}
&\tabincell{c}{3.59}
\\
\cmidrule(l){1-7}
{TF-1}
&\tabincell{c}{$0.925 \pm 0.002$}
&\tabincell{c}{$0.918 \pm 0.002$}
&\tabincell{c}{12.9}
&\tabincell{c}{3.56}
&\tabincell{c}{65.3}
&\tabincell{c}{3.50}
\\
\cmidrule(l){2-7}
{LWFT-1}
&\tabincell{c}{$0.920 \pm 0.003$}
&\tabincell{c}{$0.913 \pm 0.005$}
&\tabincell{c}{23.5}
&\tabincell{c}{4.12}
&\tabincell{c}{78.4}
&\tabincell{c}{3.55}
\\
\cmidrule(l){2-7}
{\textbf{TTL-1}}
&\tabincell{c}{\textcolor{red}{{$\mathbf{0.928 \pm 0.004}$}}}
&\tabincell{c}{\textcolor{red}{{$\mathbf{0.921 \pm 0.003}$}}}
&\tabincell{c}{{\textcolor{red}{\textbf{8.55}}}}
&\tabincell{c}{{\textcolor{red}{\textbf{3.31}}}}
&\tabincell{c}{{\textcolor{red}{\textbf{69.6}}}}
&\tabincell{c}{{\textcolor{red}{\textbf{2.99}}}}
\\


%%%%%%%%%%%%%%%%%%%%%% layer wise result
\midrule
% \parbox[t]{4mm}{\multirow{4}{*}{\rotatebox[origin=r]{90}{layer-wise}}}&

% \midrule
%\hline
% {FTL}
% &\tabincell{c}{$0.925 \pm 0.003$}
% &\tabincell{c}{$0.917 \pm 0.003$}
% &\tabincell{c}{23.5}
% &\tabincell{c}{4.12}
% &\tabincell{c}{80.1}
% &\tabincell{c}{3.59}
% \\
% \cmidrule(l){1-7}
% % &
{TF-2}
&\tabincell{c}{$0.925 \pm 0.002$}
&\tabincell{c}{$0.918 \pm 0.002$}
&\tabincell{c}{12.9}
&\tabincell{c}{3.56}
&\tabincell{c}{65.3}
&\tabincell{c}{3.50}
\\
\cmidrule(l){2-7}
% &
{LWFT-2}
&\tabincell{c}{$0.925 \pm 0.001$}
&\tabincell{c}{$0.919 \pm 0.001$}
&\tabincell{c}{23.5}
&\tabincell{c}{4.12}
&\tabincell{c}{78.2}
&\tabincell{c}{3.56}
\\
\cmidrule(l){2-7}
% &
{\textbf{TTL-2 (ours)}}
&\tabincell{c}{\textcolor{red}{{$\mathbf{0.928 \pm 0.004}$}}}
&\tabincell{c}{\textcolor{red}{{$\mathbf{0.921 \pm 0.003}$}}}
&\tabincell{c}{{\textcolor{red}{\textbf{8.55}}}}
&\tabincell{c}{{\textcolor{red}{\textbf{3.31}}}}
&\tabincell{c}{{\textcolor{red}{\textbf{69.6}}}}
&\tabincell{c}{{\textcolor{red}{\textbf{2.99}}}}

\\

\bottomrule
\end{tabular}
}}
\label{tab:mitotic_comparision_method}
% \end{center}
% \end{adjustbox}
\end{table}


